NeuRegenerate: A Framework for Visualizing Neurodegeneration

Recent advances in high-resolution microscopy have allowed scientists to better understand the underlying brain connectivity. However, due to the limitation that biological specimens can only be imaged at a single timepoint, studying changes to neural projections is limited to general observations using population analysis. In this paper, we introduce NeuRegenerate, a novel end-to-end framework for the prediction and visualization of changes in neural fiber morphology within a subject, for specified age-timepoints.To predict projections, we present neuReGANerator, a deep-learning network based on cycle-consistent generative adversarial network (cycleGAN) that translates features of neuronal structures in a region, across age-timepoints, for large brain microscopy volumes. We improve the reconstruction quality of neuronal structures by implementing a density multiplier and a new loss function, called the hallucination loss.Moreover, to alleviate artifacts that occur due to tiling of large input volumes, we introduce a spatial-consistency module in the training pipeline of neuReGANerator. We show that neuReGANerator has a reconstruction accuracy of 94% in predicting neuronal structures. Finally, to visualize the predicted change in projections, NeuRegenerate offers two modes: (1) neuroCompare to simultaneously visualize the difference in the structures of the neuronal projections, across the age timepoints, and (2) neuroMorph, a vesselness-based morphing technique to interactively visualize the transformation of the structures from one age-timepoint to the other. Our framework is designed specifically for volumes acquired using wide-field microscopy. We demonstrate our framework by visualizing the structural changes in neuronal fibers within the cholinergic system of the mouse brain between a young and old specimen.

==> full_objective.tex <==
Conclusively, the full objective for training the neuReGANerator, with cycle weights  $\Lambda_O$ and $\Lambda_Y$, is:

\begingroup
\setlength\abovedisplayskip{0.15em}
\begin{equation}
%\vspace*{-0.25em}
    \begin{split}
        \mathcal{L}_{tile}(G, F, D_O, D_Y) &= \mathcal{L}_{GAN}(F, D_O, y_{tile}, o_{tile})\\
        &+ \mathcal{L}_{GAN}(G, D_Y, o_{tile}, y_{tile})\\
        &+ \Lambda_{O} \mathcal{L}_{cyc}(G,F, o_{tile})\\
        &+ \mathcal{L}_{hallucination}(o_{tile}, y_{tile})\\
        &+ \Lambda_{Y} \mathcal{L}_{xCyc}(G,F, y_{tile})
    \end{split}
\end{equation}
\setlength\abovedisplayskip{0.15em}
\begin{equation}
%\vspace*{-0.25em}
    \begin{split}
        \mathcal{L}_{total} &= w_1\mathcal{L}_{topLeft}(G, F, D_O, D_Y)\\
        &+ w_1\mathcal{L}_{topRight}(G, F, D_O, D_Y)\\
        &+ w_1\mathcal{L}_{bottomLeft}(G, F, D_O, D_Y)\\
        &+ w_1\mathcal{L}_{bottomRight}(G, F, D_O, D_Y)\\
        &+ w_2\mathcal{L}_{center}(G, F, D_O, D_Y)
    \end{split}
\end{equation}
\endgroup
In training neuReGANerator, the network aims to solve:
\begin{equation}
    G^*,F^* = arg\: \min_{G,F}\: \max_{D_O,D_Y}\mathcal{L}(G, F, D_O, D_Y).
    %\vspace*{-0.45em}
\end{equation}
